Joint Speech Translation and Named Entity Recognition

Modern automatic translation systems aim at place the human at the center by providing contextual support and knowledge. In this context, a critical task is enriching the output with information regarding the mentioned entities, which is currently achieved processing the generated translation with named entity recognition (NER) and entity linking systems. In light of the recent promising results shown by direct speech translation (ST) models and the known weaknesses of cascades (error propagation and additional latency), in this paper we propose multitask models that jointly perform ST and NER, and compare them with a cascade baseline. The experimental results show that our models significantly outperform the cascade on the NER task (by 0.4-1.0 F1), without degradation in terms of translation quality, and with the same computational efficiency of a plain direct ST model.

==> resources/simul_plots.tex <==
\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA	CA_ONLY \\
1	18.3	0.357	1333	2795	1462 \\
2	25.4	0.414	1771	3467	1696 \\
3	30.1	0.442	2144	3962	1818 \\
%4	32.8	0.462	2491	4401	1910 \\
}\inlinesim

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA	CA_ONLY \\
1	18.5	0.356	1332	2734	1402 \\
2	25.9	0.412	1769	3435	1666 \\
3	30.5	0.446	2151	3949	1798 \\
%4	33.3	0.457	2508	4368	1861 \\
}\parallelsim

\begin{figure*}[!t]
\centering
    \begin{subfigure}[t]{0.44\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=BLEU, xlabel=ms,
            width=8cm,
            height=6cm,
            ymax=31, ymin=17,
            ytick={17,19,21,23,27,25,29,31},
            legend style={at={(1.1,1.2)},
                anchor=north,legend columns=-1},
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=BLEU]{\inlinesim};
        \addplot table[x=LAAL_CA,y=BLEU]{\parallelsim};
        \legend{Inline, Parallel + NE emb.}
    \end{axis}
\end{tikzpicture}
    \end{subfigure}
\qquad
    \begin{subfigure}[t]{0.44\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=F1, xlabel=ms,
            width=8cm,
            height=6cm,
            ymax=0.45,
            ymin=0.35,
            ytick={0.35,0.37,0.39,0.41,0.43,0.45},
            legend style={at={(1.0,1.0)},
                anchor=south,legend columns=-1},
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=F1]{\inlinesim};
        \addplot table[x=LAAL_CA,y=F1]{\parallelsim};
    \end{axis}
\end{tikzpicture} 
    \end{subfigure}
\caption{\label{fig:sim} BLEU-LAAL, and F1-LAAL curves of the \textit{inline} and \textit{parallel + NE emb} for
%\textit{k}=1,2,3 in 
en-es. All points are the average over three runs.}
\end{figure*}

==> resources/simul_plots2.tex <==
\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	18.36	0.357	1374	2300 \\
2	25.42	0.414	1817	2905 \\
3	30.08	0.442	2193	3417 \\
}\inlinees

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	19.07	0.365	1374	2249 \\
2	26.67	0.422	1817	2891 \\
3	31.36	0.456	2201	3374 \\
}\paralleles

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	19.93	0	1366	2266 \\
2	26.30	0	1784	2841 \\
3	31.07	0	2163	3342 \\
}\stes

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	27.68	0.392	1843	2854 \\
2	31.55	0.424	2223	3327 \\
3	33.64	0.439	2552	3726 \\
}\inlinefr

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	27.76	0.380	1846	2853 \\
2	31.65	0.421	2229	3333 \\
3	33.41	0.429	2560	3713 \\
}\parallelfr

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	27.52	0	1854	2869 \\
2	31.50	0	2228	3347 \\
3	33.53	0	2547	3710 \\
}\stfr

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	15.05	0.331	1334	2364 \\
2	18.91	0.364	1729	2935 \\
3	21.95	0.396	2090	3389 \\
}\inlineit

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	15.31	0.316	1360	2356 \\
2	20.11	0.378	1789	2941 \\
3	22.58	0.403	2130	3371 \\
}\parallelit

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	15.07	0	1336	2297  \\
2	19.17	0	1735	2838 \\
3	22.27	0	2106	3314 \\
}\stit

\begin{figure*}[!t]
\centering
%\hspace{0.5em}
\begin{subfigure}[t]{0.33\textwidth}
\begin{tikzpicture}
\footnotesize
\begin{axis}[
        ymajorgrids=true,
        ylabel=BLEU, xlabel=LAAL (ms),
        ytick={18,20,22,24,26,28,30,32},
        ymax=32, ymin=18,
        xmax=3500,
        ylabel shift={-2pt},
        width=6cm,
        height=6cm,
        xtick=data,
        xtick={},
    ]
    \addplot table[x=LAAL_CA,y=BLEU]{\inlinees};
    \addplot table[x=LAAL_CA,y=BLEU]{\paralleles};
    \addplot table[x=LAAL_CA,y=BLEU]{\stes};
\end{axis}
\end{tikzpicture}
\end{subfigure}
%\quad
\begin{subfigure}[t]{0.32\textwidth}
    \begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            %ylabel=BLEU, 
            xlabel=LAAL (ms),
            ytick={24,26,28,30,32,34},
            ymax=34,
            width=6cm,
            height=6cm,
            xtick=data,
            xtick={},
            legend style={at={(0.5,1.2)},%1.1,1.2
            anchor=north,legend columns=-1},
        ]
        \addplot table[x=LAAL_CA,y=BLEU]{\inlinefr};
        \addplot table[x=LAAL_CA,y=BLEU]{\parallelfr};
        \addplot table[x=LAAL_CA,y=BLEU]{\stfr};
        \legend{Inline, Parallel + NE emb., Only ST}
    \end{axis}
    \end{tikzpicture}
    \end{subfigure}
\hspace{1.3em}
\begin{subfigure}[t]{0.31\textwidth}
    \begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            %ylabel=BLEU, 
            xlabel=LAAL (ms),
            ytick={15,17,19,21,23},
            ymax=23, xmax=3500,
            width=6cm,
            height=6cm,
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=BLEU]{\inlineit};
        \addplot table[x=LAAL_CA,y=BLEU]{\parallelit};
        \addplot table[x=LAAL_CA,y=BLEU]{\stit};
    \end{axis}
    \end{tikzpicture}
    \end{subfigure}

\begin{subfigure}[t]{0.32\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=F1, xlabel=LAAL (ms),
            ytick={0.36,0.38,0.4,0.42,0.44,0.46},
            ymax=0.46, xmax=3500,
            ylabel shift={-6pt},
            width=6cm,
            height=6cm,
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=F1]{\inlinees};
        \addplot table[x=LAAL_CA,y=F1]{\paralleles};
    \end{axis}
\end{tikzpicture} 
\subcaption{en-es}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[t]{0.31\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            xlabel=LAAL (ms),
            width=6cm,
            height=6cm,
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=F1]{\inlinefr};
        \addplot table[x=LAAL_CA,y=F1]{\parallelfr};
    \end{axis}
\end{tikzpicture} 
\subcaption{en-fr}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[t]{0.31\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            xlabel=LAAL (ms),
            ytick={0.31,0.33,0.35,0.37,0.39,0.41},
            ymax=0.41, ymin=0.31,
            xmax=3500,
            width=6cm,
            height=6cm,
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=F1]{\inlineit};
        \addplot table[x=LAAL_CA,y=F1]{\parallelit};
    \end{axis}
\end{tikzpicture} 
\subcaption{en-it}
\end{subfigure}
\caption{\label{fig:sim} BLEU-LAAL, and F1-LAAL curves of the \textit{inline} and \textit{parallel + NE emb} models for en-es, en-fr, and en-it. 
%All points are 
\sara{Each point corresponds to a different value of $k=\{1,2,3\}$ and is}
the average over three runs.}
\end{figure*}

==> resources/simul_plots3.tex <==
\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA	CA_ONLY \\
1	18.3	0.357	1333	2795	1462 \\
2	25.4	0.414	1771	3467	1696 \\
3	30.1	0.442	2144	3962	1818 \\
%4	32.8	0.462	2491	4401	1910 \\
}\inlinesim

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA	CA_ONLY \\
1	18.5	0.356	1332	2734	1402 \\
2	25.9	0.412	1769	3435	1666 \\
3	30.5	0.446	2151	3949	1798 \\
%4	33.3	0.457	2508	4368	1861 \\
}\parallelsim

\begin{figure}[!t]
\centering
\quad
    \begin{subfigure}[t]{0.45\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=BLEU, xlabel=LAAL (ms),
            width=8cm,
            height=5cm,
            ymax=31, ymin=17,
            ytick={17,19,21,23,27,25,29,31},
            legend style={at={(0.5,1.2)},
                anchor=north,legend columns=-1},
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=BLEU]{\inlinesim};
        \addplot table[x=LAAL_CA,y=BLEU]{\parallelsim};
        \legend{Inline, Parallel + NE emb.}
    \end{axis}
\end{tikzpicture}
    \end{subfigure}
\\
%\qquad
    \begin{subfigure}[t]{0.45\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=F1, xlabel=LAAL (ms),
            width=8cm,
            height=5cm,
            ymax=0.45,
            ymin=0.35,
            ytick={0.35,0.37,0.39,0.41,0.43,0.45},
            legend style={at={(1.0,1.0)},
                anchor=south,legend columns=-1},
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=F1]{\inlinesim};
        \addplot table[x=LAAL_CA,y=F1]{\parallelsim};
    \end{axis}
\end{tikzpicture} 
    \end{subfigure}
\caption{\label{fig:sim} BLEU-LAAL, and F1-LAAL curves of the \textit{inline} and \textit{parallel + NE emb} for en-es. \sara{Each point corresponds to a different value of $k=\{1,2,3\}$ and is}
the average over three runs.}
\end{figure}

==> resources/simul_plots4.tex <==
\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	18.36	0.357	1374	2300 \\
2	25.42	0.414	1817	2905 \\
3	30.08	0.442	2193	3417 \\
}\inlinesim

\pgfplotstableread[row sep=\\]{
k	BLEU	F1	LAAL	LAAL_CA \\
1	19.07	0.365	1374	2249 \\
2	26.67	0.422	1817	2891 \\
3	31.36	0.456	2201	3374 \\
}\parallelsim

\begin{figure}[!t]
\centering
\quad
    \begin{subfigure}[t]{0.45\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=BLEU, xlabel=ms,
            width=8cm,
            height=5cm,
            ymax=31, ymin=17,
            ytick={17,19,21,23,27,25,29,31},
            legend style={at={(0.5,1.2)},
                anchor=north,legend columns=-1},
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=BLEU]{\inlinesim};
        \addplot table[x=LAAL_CA,y=BLEU]{\parallelsim};
        \legend{Inline, Parallel + NE emb.}
    \end{axis}
\end{tikzpicture}
    \end{subfigure}
\\
%\qquad
    \begin{subfigure}[t]{0.45\textwidth}
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
            ymajorgrids=true,
            ylabel=F1, xlabel=ms,
            width=8cm,
            height=5cm,
            ymax=0.45,
            ymin=0.35,
            ytick={0.35,0.37,0.39,0.41,0.43,0.45},
            legend style={at={(1.0,1.0)},
                anchor=south,legend columns=-1},
            xtick=data,
            xtick={},
        ]
        \addplot table[x=LAAL_CA,y=F1]{\inlinesim};
        \addplot table[x=LAAL_CA,y=F1]{\parallelsim};
    \end{axis}
\end{tikzpicture} 
    \end{subfigure}
\caption{\label{fig:sim} BLEU-LAAL, and F1-LAAL curves of the \textit{inline} and \textit{parallel + NE emb} for
%\textit{k}=1,2,3 in 
en-es. 
%All 
\sara{Each point corresponds to a different value of $k=\{1,2,3\}$ and is}
%points are 
the average over three runs.}
\end{figure}
